Upgrading the protection of children from manipulative and addictive strategies in online games: Legal and technical solutions beyond privacy regulation

Despite the increasing awareness from academia, civil society and media to the issue of child manipulation online, the current EU regulatory system fails at providing sufficient levels of protection. Given the universality of the issue, there is a need to combine and further these scattered efforts into a unitary, multidisciplinary theory of digital manipulation that identifies causes and effects, systematizes the technical and legal knowledge on manipulative and addictive tactics, and to find effective regulatory mechanisms to fill the legislative gaps. In this paper we discuss manipulative and exploitative strategies in the context of online games for children, suggest a number of possible reasons for the failure of the applicable regulatory system, propose an "upgrade" for the regulatory approach to address these risks from the perspective of freedom of thought, and present and discuss technological approaches that allow for the development of games that verifiably protect the privacy and freedoms of players.

==> refs.tex <==

\subsection*{References}

Acquisti, Alessandro, Idris Adjerid, Rebecca Balebako, Laura
Brandimarte, Lorrie Faith Cranor, Saranga Komanduri, Pedro Giovanni
Leon, et al. 2017. ``Nudges for Privacy and Security: Understanding and
Assisting Users' Choices Online.'' ACM Computing Surveys (CSUR) 50 (3):
1--41.\protect\hypertarget{anchor-25}{}{}

Alha, Kati. "The rise of free-to-play: How the revenue model changed
games and playing." (2020).

Alegre, Susie. 2021a. ``Protecting Freedom of Thought in the Digital
Age.''\protect\hypertarget{anchor-26}{}{}

---------. 2021b. ``Regulating Around Freedom in the `Forum Internum'.''
In ERA Forum, 21:591--604. 4.
Springer.\protect\hypertarget{anchor-27}{}{}

Arrington, Robert L. 1982. ``Advertising and Behavior Control.'' Journal
of Business Ethics 1 (1): 3--12.\protect\hypertarget{anchor-28}{}{}

Aylsworth, Timothy. 2020. ``Autonomy and Manipulation: Refining the
Argument Against Persuasive Advertising.'' Journal of Business Ethics,
1--11.\protect\hypertarget{anchor-29}{}{}

Baker, Sherry, and David L Martinson. 2001. ``The Tares Test: Five
Principles for Ethical Persuasion.'' Journal of Mass Media Ethics 16
(2-3): 148--75.\protect\hypertarget{anchor-30}{}{}

Barocas, Solon, and Helen Nissenbaum. 2009. ``On Notice: The Trouble
with Notice and Consent.'' In Proceedings of the Engaging Data Forum:
The First International Forum on the Application and Management of
Personal Electronic Information.\protect\hypertarget{anchor-31}{}{}

Ben-Shahar, Omri, and Carl E Schneider. 2014. More Than You Wanted to
Know: The Failure of Mandated Disclosure. Princeton University
Press.\protect\hypertarget{anchor-32}{}{}

Blades, Mark, Caroline Oates, Fran Blumberg, and Barrie Gunter. 2014.
Advertising to Children: New Directions, New Media. Springer.

Blumberg, F. C., Deater-Deckard, K., Calvert, S. L., Flynn, R. M.,
Green, C. S., Arnold, D., \& Brooks, P. J. (2019). Digital Games as a
Context for Children's Cognitive Development: Research Recommendations
and Policy Considerations. Social Policy Report, 32(1), 1--33.

Brownsword, Roger. 2012. ``Regulating Brain Imaging: Questions of
Privacy, Informed Consent, and Human Dignity.'' I Know What You're
Thinking. Brain Imaging and Mental Privacy. Oxford University Press,
Oxford, 223--44.\protect\hypertarget{anchor-33}{}{}

Bublitz, Jan-Christoph. 2013. ``My Mind Is Mine!? Cognitive Liberty as a
Legal Concept.'' In Cognitive Enhancement, 233--64.
Springer.\protect\hypertarget{anchor-34}{}{}

Candy, Peter. 2018. ``Lex (P) Laetoria.'' In Oxford Research
Encyclopedia of Classics.\protect\hypertarget{anchor-35}{}{}

Canli, Turhan. 2006. ``When Genes and Brains Unite: Ethical Implications
of Genomic Neuroimaging.'' Neuroethics: Defining the Issues in Theory,
Practice and Policy, 169--84.\protect\hypertarget{anchor-36}{}{}

Carr, Nicholas. 2020. The Shallows: What the Internet Is Doing to Our
Brains. WW Norton \& Company.\protect\hypertarget{anchor-37}{}{}

Chatterjee, Rahul, Periwinkle Doerfler, Hadas Orgad, Sam Havron,
Jackeline Palmer, Diana Freed, Karen Levy, Nicola Dell, Damon McCoy, and
Thomas Ristenpart. 2018. ``The Spyware Used in Intimate Partner
Violence.'' In 2018 Ieee Symposium on Security and Privacy (Sp),
441--58. IEEE.\protect\hypertarget{anchor-38}{}{}

Clarke, Barbie, and Siv Svanaes. 2012. ``Digital Marketing and
Advertising to Children: A Literature Review.'' In Advertising Education
Forum. Vol. 79.\protect\hypertarget{anchor-39}{}{}

Commons, House of. 2019. ``Immersive and Addictive
Technologies.''\protect\hypertarget{anchor-40}{}{}

Council, Norwegian Consumer. 2018. ``Deceived by Design, How Tech
Companies Use Dark Patterns to Discourage Us from Exercising Our Rights
to Privacy.'' Norwegian Consumer Council
Report.\protect\hypertarget{anchor-41}{}{}

Council of Europe, Parliamentary Assembly. 2017. ``Technological
Convergence, Artificial Intelligence and Human Rights.''

Crepax, T., Muntés-Mulero, V., Martinez, J., \& Ruiz, A. (2022).
Information technologies exposing children to privacy risks: Domains and
children-specific technical controls. Computer Standards \& Interfaces,
82, 103624

Crisp, Roger. 1987. ``Persuasive Advertising, Autonomy, and the Creation
of Desire.'' Journal of Business Ethics 6 (5):
413--18.\protect\hypertarget{anchor-42}{}{}

Dalla Corte, Lorenzo. 2020. ``A Right to a Rule: On the Substance and
Essence of the Fundamental Right to Personal Data Protection.'' Data
Protection and Privacy, 27--58.\protect\hypertarget{anchor-43}{}{}

De Jans, Steffi, Dieneke Van de Sompel, Liselot Hudders, and Veroline
Cauberghe. 2019. ``Advertising Targeting Young Children: An Overview of
10 Years of Research (2006--2016).'' International Journal of
Advertising 38 (2): 173--206.\protect\hypertarget{anchor-44}{}{}

Demmler, Daniel, Peter Rindal, Mike Rosulek, and Ni Trieu. 2018.
``PIR-Psi: Scaling Private Contact Discovery.'' Proc. Priv. Enhancing
Technol. 2018 (4): 159--78.

Drummond, A., \& Sauer, J. D. (2018). Video game loot boxes are
psychologically akin to gambling. Nature Human Behaviour, 2(8),
530--532.\protect\hypertarget{anchor-45}{}{}Duch-Brown, Nestor, Bertin
Martens, and Frank Mueller-Langer. 2017. ``The Economics of Ownership,
Access and Trade in Digital Data.''\protect\hypertarget{anchor-46}{}{}

Durante, Kristina M, Vladas Griskevicius, Sarah E Hill, Carin Perilloux,
and Norman P Li. 2011. ``Ovulation, Female Competition, and Product
Choice: Hormonal Influences on Consumer Behavior.'' Journal of Consumer
Research 37 (6): 921--34.\protect\hypertarget{anchor-47}{}{}

El-Nasr, Magy Seif, Anders Drachen, and Alessandro Canossa. Game
analytics. Springer London Limited, 2016.

Europe, Council of. 2019. ``Declaration by the Committee of Ministers on
the Manipulative Capabilities of Algorithmic
Processes.''\protect\hypertarget{anchor-48}{}{}

Fenton, Ted, and Reinout W Wiers. 2017. ``Free Will, Black Swans and
Addiction.'' Neuroethics 10 (1): 157--65.

Fitton, D., \& Read, J. C. (2019, June). Creating a framework to support
the critical consideration of dark design aspects in free-to-play apps.
In Proceedings of the 18th ACM International Conference on Interaction
Design and Children (pp. 407-418).

Fischbach, Ruth, and Janet Mindes. 2011. ``Why Neuroethicists Are
Needed.'' Oxford Handbook of Neuroethics,
343--76.\protect\hypertarget{anchor-49}{}{}

Fogg, Brian J. 2002. ``Persuasive Technology: Using Computers to Change
What We Think and Do.'' Ubiquity 2002 (December):
2.\protect\hypertarget{anchor-50}{}{}

Ford, John B. 2019. ``What Do We Know About Neuromarketing?'' Journal of
Advertising Research.
\url{https://doi.org/10.2501/JAR-2019-031}.\protect\hypertarget{anchor-51}{}{}

Fukuyama, Francis. 2003. Our Posthuman Future: Consequences of the
Biotechnology Revolution. Farrar, Straus;
Giroux.\protect\hypertarget{anchor-52}{}{}

Gilbert, Neil, Nigel Parton, and Marit Skivenes. 2011. Child Protection
Systems: International Trends and Orientations. OUP
USA.\protect\hypertarget{anchor-53}{}{}

Greene, Joshua, and Jonathan Cohen. 2004. ``For the Law, Neuroscience
Changes Nothing and Everything.'' Philosophical Transactions of the
Royal Society of London. Series B: Biological Sciences 359 (1451):
1775--85.\protect\hypertarget{anchor-54}{}{}

Griffiths, Mark D. "Adolescent gambling and gambling-type games on
social networking sites: Issues, concerns, and recommendations." Aloma:
revista de psicologia, ciències de l'educació i de l'esport Blanquerna
33, no. 2 (2015): 31-37.

Hargittai, Eszter, and Alice Marwick. "``What can I really do?''
Explaining the privacy paradox with online apathy." International
journal of communication 10 (2016): 21.

Harris, Tristan. 2016. ``How Technology Hijacks People's Minds---from a
Magician and Google's Design Ethicist.'' Medium
Magazine.\protect\hypertarget{anchor-55}{}{}

Hartzog, Woodrow. 2018. Privacy's Blueprint: The Battle to Control the
Design of New Technologies. Harvard University
Press.\protect\hypertarget{anchor-56}{}{}

Hullett, Kenneth, Nagappan, Nachiappan, Schuh, Eric, and Hopson, John.
"Empirical analysis of user data in game software development,"
Proceedings of the 2012 ACM-IEEE International Symposium on Empirical
Software Engineering and Measurement, 2012, pp. 89-98, doi:
10.1145/2372251.2372265.

Ienca, Marcello, and Roberto Andorno. 2017. ``Towards New Human Rights
in the Age of Neuroscience and Neurotechnology.'' Life Sciences, Society
and Policy 13 (1): 1--27.\protect\hypertarget{anchor-57}{}{}

Ienca, Marcello, and Gianclaudio Malgieri. 2021. ``Mental Data
Protection and the Gdpr.'' Available at SSRN
3840403.\protect\hypertarget{anchor-58}{}{}

Kales, Daniel, Christian Rechberger, Thomas Schneider, Matthias Senker,
and Christian Weinert. 2019. ``Mobile Private Contact Discovery at
Scale.'' In 28th USENIX Security Symposium (USENIX Security 19),
1447--64.

Karlsen, F. (2020). Game Creation, Monetisation Models, and Ethical
Concerns.

Karlsen, F. (2021). Balancing Ethics, Art and Economics: A Qualitative
Analysis of Game Designer Perspectives on Monetisation. Games and
Culture, 15554120211049579.Kenning, Peter, and Marc Linzmajer. 2011.
``Consumer Neuroscience: An Overview of an Emerging Discipline with
Implications for Consumer Policy.'' Journal Für Verbraucherschutz Und
Lebensmittelsicherheit 6 (1): 111--25.

King, D. L., \& Delfabbro, P. H. (2018). Predatory monetization schemes
in video games (eg `loot boxes') and internet gaming
disorder.\protect\hypertarget{anchor-59}{}{}

Kidron, Beeban, Alexandra Evans, Jenny Afia, Joanna R Adler, Henrietta
Bowden-Jones, Liam Hackett, Anisha Juj, Andrew K Przybylski, Anghrarad
Rudkin, and Young Scot. 2018. ``Disrupted Childhood: The Cost of
Persuasive Design.''\protect\hypertarget{anchor-60}{}{}

Király, Orsolya, Mark D Griffiths, Daniel L King, Hae-Kook Lee,
Seung-Yup Lee, Fanni Bányai, Ágnes Zsila, Zsofia K Takacs, and Zsolt
Demetrovics. 2018. ``Policy Responses to Problematic Video Game Use: A
Systematic Review of Current Measures and Future Possibilities.''
Journal of Behavioral Addictions 7 (3):
503--17.\protect\hypertarget{anchor-61}{}{}

Koob, George F, and Nora D Volkow. 2016. ``Neurobiology of Addiction: A
Neurocircuitry Analysis.'' The Lancet Psychiatry 3 (8):
760--73.\protect\hypertarget{anchor-62}{}{}

Kröger, Jacob Leon, Philip Raschke, Jessica Percy Campbell, and Stefan
Ullrich. 2021. ``Surveilling the Gamers: Privacy Impacts of the Video
Game Industry.'' Available at SSRN
3881279.\protect\hypertarget{anchor-63}{}{}

LaRose, Robert, and Nora J Rifon. 2007. ``Promoting I-Safety: Effects of
Privacy Warnings and Privacy Seals on Risk Assessment and Online Privacy
Behavior.'' Journal of Consumer Affairs 41 (1):
127--49.\protect\hypertarget{anchor-64}{}{}

Laufer, Robert S, and Maxine Wolfe. 1977. ``Privacy as a Concept and a
Social Issue: A Multidimensional Developmental Theory.'' Journal of
Social Issues 33 (3): 22--42.\protect\hypertarget{anchor-65}{}{}

Leshner, Alan I. 1997. ``Addiction Is a Brain Disease, and It Matters.''
Science 278 (5335): 45--47.\protect\hypertarget{anchor-66}{}{}

Lessig, Lawrence. 2009. Code: And Other Laws of Cyberspace.
ReadHowYouWant. com.\protect\hypertarget{anchor-67}{}{}

Lievens, Eva, Sonia Livingstone, Sharon McLaughlin, Brian O'Neill, and
Valerie Verdoodt. 2018. ``Children's Rights and Digital Technologies.''
International Children's Rights Law,
487--513.\protect\hypertarget{anchor-68}{}{}

Lindstrom, Martin. 2010. Buy Ology: Truth and Lies About Why We Buy.
Currency.\protect\hypertarget{anchor-69}{}{}

Livingstone, Sonia, John Carr, and Jasmina Byrne. 2016. ``One in Three:
Internet Governance and Children's
Rights.''\protect\hypertarget{anchor-70}{}{}

Livingstone, Sonia, Mariya Stoilova, and Rishita Nandagiri. 2018.
``Conceptualising Privacy Online: What Do, and What Should, Children
Understand?'' Parenting for a Digital
Future.\protect\hypertarget{anchor-71}{}{}

---------. 2019. ``Children's Data and Privacy Online: Growing up in a
Digital Age: An Evidence Review.''\protect\hypertarget{anchor-72}{}{}

Livingstone, Sonia, Damian Tambini, Nikola Belakova, and Emma Goodman.
2018. ``Protection of Children Online: Does Current Regulation
Deliver?''\protect\hypertarget{anchor-73}{}{}

Lupton, Deborah, and Ben Williamson. 2017. ``The Datafied Child: The
Dataveillance of Children and Implications for Their Rights.'' New Media
\& Society 19 (5): 780--94.\protect\hypertarget{anchor-74}{}{}

Lwin, May O., Andrea JS Stanaland, and Anthony D. Miyazaki. "Protecting
children's privacy online: How parental mediation strategies affect
website safeguard effectiveness." Journal of retailing 84, no. 2 (2008):
205-217.

Macenaite, Milda, and Eleni Kosta. 2017. ``Consent for Processing
Children's Personal Data in the Eu: Following in Us Footsteps?''
Information \& Communications Technology Law 26 (2):
146--97.\protect\hypertarget{anchor-75}{}{}

Madigan, Jamie. 2015. Getting Gamers: The Psychology of Video Games and
Their Impact on the People Who Play Them. Rowman \&
Littlefield.\protect\hypertarget{anchor-76}{}{}

Maene, P., J. Götzfried, R. de Clercq, T. Müller, F. Freiling, and I.
Verbauwhede. 2017. ``Hardware-Based Trusted Computing Architectures for
Isolation and Attestation.'' IEEE Transactions on Computers PP (99):
1--1.\protect\hypertarget{anchor-77}{}{}

Matthews, Steve. 2015. ``Neuromarketing: What is it and is it a threat
to privacy?'' In Handbook of Neuroethics.
\url{https://doi.org/10.1007/978-94-007-4707-4_154}.\protect\hypertarget{anchor-78}{}{}

McCarthy-Jones, Simon. 2019. ``The Autonomous Mind: The Right to Freedom
of Thought in the Twenty-First Century.'' Frontiers in Artificial
Intelligence 2: 19.

Melzer, A. K., Roarsen, A. K., Hagen, M. H., \& Jaccheri, L. (2021,
November). Towards Suitable Free-to-Play Games for Children. In
International Conference on Entertainment Computing (pp. 264-276).
Springer, Cham.

moxie0. 2017. ``Technology Preview: Private Contact Discovery for
Signal.''\protect\hypertarget{anchor-79}{}{}

Murphy, Emily R, Judy Illes, and Peter B Reiner. 2008. ``Neuroethics of
Neuromarketing.'' Journal of Consumer Behaviour: An International
Research Review 7 (4-5): 293--302.\protect\hypertarget{anchor-80}{}{}

Newman, Joe, and Joseph Jerome. 2014. ``Press Start to Track Privacy and
the New Questions Posed by Modern Video Game Technology.'' AIPLA QJ 42:
527.\protect\hypertarget{anchor-81}{}{}

OECD. 2021. ``Children in the Digital Environment,'' no. 302.
\href{https://doi.org/https:/doi.org/https:/doi.org/10.1787/9b8f222e-en}{https://doi.org/https://doi.org/https://doi.org/10.1787/9b8f222e-en}.\protect\hypertarget{anchor-82}{}{}

O'Keeffe, Gwenn Schurgin, Kathleen Clarke-Pearson, and others. 2011.
``The Impact of Social Media on Children, Adolescents, and Families.''
Pediatrics 127 (4): 800--804.\protect\hypertarget{anchor-83}{}{}

Onnela, Jukka-Pekka, and Scott L Rauch. 2016. ``Harnessing
Smartphone-Based Digital Phenotyping to Enhance Behavioral and Mental
Health.'' Neuropsychopharmacology 41 (7):
1691--6.\protect\hypertarget{anchor-84}{}{}

Owen, Laura, Charlie Lewis, Susan Auty, and Moniek Buijzen. 2013. ``Is
Children's Understanding of Nontraditional Advertising Comparable to
Their Understanding of Television Advertising?'' Journal of Public
Policy \& Marketing 32 (2): 195--206.\protect\hypertarget{anchor-85}{}{}

Pasquale, Liliana, and Paola Zippo. 2020. ``A Review of Age Verification
Mechanism for 10 Social Media Apps.''\protect\hypertarget{anchor-86}{}{}

Purtova, Nadezhda. 2018. ``The Law of Everything. Broad Concept of
Personal Data and Future of Eu Data Protection Law.'' Law, Innovation
and Technology 10 (1): 40--81.\protect\hypertarget{anchor-87}{}{}

Ramsøy, Thomas Zoëga. 2019. ``Building a Foundation for Neuromarketing
and Consumer Neuroscience Research: How Researchers Can Apply Academic
Rigor to the Neuroscientific Study of Advertising Effects.'' Journal of
Advertising Research 59 (3): 281--94.\protect\hypertarget{anchor-88}{}{}

Ringland, Kathryn E. 2019. ```Autsome': Fostering an Autistic Identity
in an Online Minecraft Community for Youth with Autism.'' In
International Conference on Information, 132--43.
Springer.\protect\hypertarget{anchor-89}{}{}

Russell, N Cameron, Joel R Reidenberg, and Sumyung Moon. 2018. ``Privacy
in Gaming.'' Fordham Intell. Prop. Media \%Ent. LJ 29:
61.\protect\hypertarget{anchor-90}{}{}

Sartor, Giovanni, Francesca Lagioia, and Federico Galli. 2021.
``Regulating Targeted and Behavioural Advertising in Digital
Services.''\protect\hypertarget{anchor-91}{}{}

Sax, Marijn, and Jef Ausloos. 2021. ``Getting Under Your Skin(s): A
Legal-Ethical Exploration of Fortnite's Transformation into a Content
Delivery Platform and Its Manipulative Potential.'' Interactive
Entertainment Law Review 4 (1).\protect\hypertarget{anchor-92}{}{}

Schaik, Stephan van, Andrew Kwong, Daniel Genkin, and Yuval Yarom. 2020.
``SGAxe: How SGX Fails in Practice.''\protect\hypertarget{anchor-93}{}{}

Schaub, Florian, Rebecca Balebako, Adam L Durity, and Lorrie Faith
Cranor. 2015. ``A Design Space for Effective Privacy Notices.'' In
Eleventh Symposium on Usable Privacy and Security
(
\todo[inline]{figure!}
%
%\includegraphics[width=0.041cm,height=0.467cm]{./ObjectReplacements/Object 2}
%
Soups
\todo[inline]{figure!}
%
%\includegraphics[width=0.041cm,height=0.467cm]{./ObjectReplacements/Object 4}
%
2015), 1--17.\protect\hypertarget{anchor-94}{}{}

Schüll, Natasha Dow. 2012. Addiction by Design. Princeton University
Press.\protect\hypertarget{anchor-95}{}{}

Schultz, Wolfram, Peter Dayan, and P Read Montague. 1997. ``A Neural
Substrate of Prediction and Reward.'' Science 275 (5306):
1593--9.\protect\hypertarget{anchor-96}{}{}

Scopelliti, Gianluca, Sepideh Pouyanrad, Job Noorman, Fritz Alder, Frank
Piessens, and Jan Tobias Mühlberg. 2021. ``POSTER: An Open-Source
Framework for Developing Heterogeneous Distributed Enclave
Applications.'' In CCS '21. New York, NY, USA: ACM.
\url{https://doi.org/10.1145/3460120.3485341}.\protect\hypertarget{anchor-97}{}{}

Sententia, Wrye. 2004. ``Neuroethical Considerations: Cognitive Liberty
and Converging Technologies for Improving Human Cognition.'' Annals of
the New York Academy of Sciences 1013 (1):
221--28.\protect\hypertarget{anchor-98}{}{}

Sher, Shlomo. 2011. ``A Framework for Assessing Immorally Manipulative
Marketing Tactics.'' Journal of Business Ethics 102 (1):
97--118.\protect\hypertarget{anchor-99}{}{}

Sieber, Alexander. 2019. ``Souled out of rights? - Predicaments in
protecting the human spirit in the age of neuromarketing.'' In Life
Sciences, Society and Policy. Vol. 15. 1.
\url{https://doi.org/10.1186/s40504-019-0095-4}.\protect\hypertarget{anchor-100}{}{}

Sifa, Rafet, Anders Drachen, and Christian Bauckhage. 2018. ``Profiling
in Games: Understanding Behavior from Telemetry.'' Social Interactions
in Virtual Worlds: An Interdisciplinary
Perspective.\protect\hypertarget{anchor-101}{}{}

signal. 2021. ``Signal.''\protect\hypertarget{anchor-102}{}{}

Simon, Herbert A. 1994. ``The Bottleneck of Attention: Connecting
Thought with Motivation.''\protect\hypertarget{anchor-103}{}{}

Skriabin, Oleksii M, Dmytro B Sanakoiev, Natalia D Sanakoieva, Vita V
Berezenko, and Yuliia V Liubchenko. 2021. ``Neurotechnologies in the
advertising industry: Legal and ethical aspects.'' Innovative Marketing
17 (2): 2021.
\url{https://doi.org/10.21511/im.17(2).2021.17}.\protect\hypertarget{anchor-104}{}{}

Sloan, Robert H, and Richard Warner. 2014. ``Beyond Notice and Choice:
Privacy, Norms, and Consent.'' J. High Tech. L. 14:
370.\protect\hypertarget{anchor-105}{}{}

Small, Gary W, Jooyeon Lee, Aaron Kaufman, Jason Jalil, Prabha Siddarth,
Himaja Gaddipati, Teena D Moody, and Susan Y Bookheimer. 2020. ``Brain
Health Consequences of Digital Technology Use.'' Dialogues in Clinical
Neuroscience 22 (2): 179.\protect\hypertarget{anchor-106}{}{}

Smidts, Ale. 2002. ``Kijken in Het Brein: Over de Mogelijkheden van
Neuromarketing.''\protect\hypertarget{anchor-107}{}{}

Smith, Karen Louise, and Leslie Regan Shade. "Children's digital
playgrounds as data assemblages: Problematics of privacy,
personalization, and promotional culture." Big Data \& Society 5, no. 2
(2018): 2053951718805214.

Stanton, Steven J, Walter Sinnott-Armstrong, and Scott A Huettel. 2017.
``Neuromarketing: Ethical Implications of Its Use and Potential
Misuse.'' Journal of Business Ethics 144 (4):
799--811.\protect\hypertarget{anchor-108}{}{}

Steeves, Valerie, and Cheryl Webster. "Closing the barn door: The effect
of parental supervision on Canadian children's online privacy." Bulletin
of Science, Technology \& Society 28, no. 1 (2008): 4-19.

Su, Yanhui, Per Backlund, and Henrik Engström. "Comprehensive review and
classification of game analytics." Service Oriented Computing and
Applications 15, no. 2 (2021): 141-156.

Suleman, Muhammad, Tariq Rahim Soomro, Taher M Ghazal, and Muhammad
Alshurideh. 2021. ``Combating Against Potentially Harmful Mobile Apps.''
In The International Conference on Artificial Intelligence and Computer
Vision, 154--73. Springer.\protect\hypertarget{anchor-109}{}{}

Swan, Melanie. 2012. ``Sensor Mania! The Internet of Things, Wearable
Computing, Objective Metrics, and the Quantified Self 2.0.'' Journal of
Sensor and Actuator Networks 1 (3):
217--53.\protect\hypertarget{anchor-110}{}{}

Third, Amanda, Delphine Bellerose, Juliano Diniz De Oliveira, Girish
Lala, and Georgina Theakstone. 2017. ``Young and Online: Children's
Perspectives on Life in the Digital
Age.''\protect\hypertarget{anchor-111}{}{}

Van den Berg, Bibi, and Simone Van der Hof. 2012. ``What Happens to My
Data? A Novel Approach to Informing Users of Data Processing
Practices.'' First Monday 17 (7).\protect\hypertarget{anchor-112}{}{}

Simone, van der Hof, and Eva Lievens. "The importance of privacy by
design and data protection impact assessments in strengthening
protection of children's personal data under the GDPR." Communications
law 23, no. 1 (2018).

Van Reijmersdal, Eva A, Jeroen Jansz, Oscar Peters, and Guda Van Noort.
2010. ``The Effects of Interactive Brand Placements in Online Games on
Children's Cognitive, Affective, and Conative Brand Responses.''
Computers in Human Behavior 26 (6):
1787--94.\protect\hypertarget{anchor-113}{}{}

Verdoodt, Valerie. 2020. Children's Rights and Commercial Communication
in the Digital Era. Vol. 10.
Intersentia.\protect\hypertarget{anchor-114}{}{}

Waiguny, Martin KJ, Michelle R Nelson, and Ralf Terlutter. 2014. ``The
Relationship of Persuasion Knowledge, Identification of Commercial
Intent and Persuasion Outcomes in Advergames---the Role of Media Context
and Presence.'' Journal of Consumer Policy 37 (2):
257--77.\protect\hypertarget{anchor-115}{}{}

Wardlaw, Joanna M, Garret O'connell, Kirsten Shuler, Janet DeWilde, Jane
Haley, Oliver Escobar, Shaun Murray, et al. 2011. ```Can It Read My
Mind?'--What Do the Public and Experts Think of the Current (Mis) Uses
of Neuroimaging?'' PloS One 6 (10):
e25829.\protect\hypertarget{anchor-116}{}{}

Wilson, Edward O. 2017. The Origins of Creativity. Liveright
Publishing.\protect\hypertarget{anchor-117}{}{}

Wilson, R Mark, Jeannie Gaines, and Ronald Paul Hill. 2008.
``Neuromarketing and Consumer Free Will.'' Journal of Consumer Affairs
42 (3): 389--410.\protect\hypertarget{anchor-118}{}{}

Wright, Benjamin D. 1997. ``A History of Social Science Measurement.''
Educational Measurement: Issues and Practice 16 (4):
33--45.\protect\hypertarget{anchor-119}{}{}

Wu, Tim. 2017. The Attention Merchants: The Epic Scramble to Get Inside
Our Heads. Vintage.\protect\hypertarget{anchor-120}{}{}

Wuyts, Kim, Laurens Sion, and Wouter Joosen. 2020. ``LINDDUN Go: A
Lightweight Approach to Privacy Threat Modeling.'' In 2020 Ieee European
Symposium on Security and Privacy Workshops (Euros\&PW), 302--9.
IEEE.\protect\hypertarget{anchor-121}{}{}

Zuboff, Shoshana. 2019. ``Surveillance Capitalism.'' Esprit 5: 63--77.


==> summary.tex <==
Many online video games are designed to be manipulative, addictive
personal data collection machines. Free-to-play (F2P) mobile games (or
\enquote{freemiums}) exploit established and novel marketing techniques to
take advantage of users' weaknesses, nudging them into in-app purchasing
of items, and perpetually seek the user's attention.
 
A substantial portion of freemium consumers are represented by children.
Most prominently during middle childhood, children are exceptionally
vulnerable to such covert, manipulative marketing tactics and, unaware
of the risks that seemingly harmless online games pose to their
fundamental rights, they often fall prey to addictive behaviors that put
their health and well-being in jeopardy. A current trend in marketing,
which is informed by neuroscientific knowledge, boosted by data
analytics and machine learning techniques, interferes with children's
self-determination and development, health and social life in ways that
should undergo renewed legal and ethical scrutiny.
 
To such imminent threats, the practical implementations in the EU of
human rights, consumer protection and digital services regulation, have
failed the test of digital reality -- mostly, due to a general fixation
on regulation based on notice and consent, overestimation of supervisory
authorities capabilities and underestimation of effects on children.
Meanwhile, the EU's latest regulatory efforts, although overall more
aware of the manipulation issue, will only exercise their effects
sometimes in the distant future.
 
Despite the increasing awareness from academia, civil society and media
to the issue of child manipulation online, the current EU regulatory
system fails at providing sufficient levels of protection. In this paper
we discuss manipulative and exploitative strategies in the context of
online games for children, suggest a number of possible reasons for the
failure of the applicable regulatory system, propose an \enquote{upgrade} for
the regulatory approach to address these risks from the perspective of
freedom of thought, and present and discuss technological approaches
that allow for the development of games that verifiably protect the
privacy and freedoms of players.


